Counterfactual-Consistency Prompting for Relative Temporal Understanding in Large Language Models

Despite the advanced capabilities of large language models (LLMs), their temporal reasoning ability remains underdeveloped. Prior works have highlighted this limitation, particularly in maintaining temporal consistency when understanding events. For example, models often confuse mutually exclusive temporal relations like ``before'' and ``after'' between events and make inconsistent predictions. In this work, we tackle the issue of temporal inconsistency in LLMs by proposing a novel counterfactual prompting approach. Our method generates counterfactual questions and enforces collective constraints, enhancing the model's consistency. We evaluate our method on multiple datasets, demonstrating significant improvements in event ordering for explicit and implicit events and temporal commonsense understanding by effectively addressing temporal inconsistencies.

==> tables/contrast_examples.tex <==


\begin{table*}[h]
\centering
\scalebox{0.82}{
\begin{tabular}{|l|l|l|l|}
\hline
 \textbf{Dataset} & \textbf{Relation} & \textbf{Revision Type} & \textbf{Example} \\ \hline
 TempEvalBi-QA \& TRACIE & $r_1(e_1,e_2)$ & Original & They got married \textbf{after} they moved to Maine. \\ 
 & $r_2(e_1,e_2)$ & $r_1 \rightarrow r_2$ & They got married \textbf{before} they moved to Maine. \\ \hline
 MCTACO: Ordering & $r_1(e_1,e_2)$ & Original & They \textbf{went to the store} after they were put in jail. \\ 
& $r_1(e_1,e_3)$ & $e_2 \rightarrow e_3$ & They \textbf{repented} after they were put in jail. \\ \hline
 MCTACO: Duration, & $r_1(e_1)$ & Original & It has existed for \textbf{1 year}. \\ 
 Frequency, Typical Time  & $r_2(e_1)$ & $r_1 \rightarrow r_2$ & It has existed for \textbf{centuries}. \\ \hline
 MCTACO: Stationarity & $r_1(e_1)$ & Original & She is \textbf{still} in Ranchipur. \\  
& $\neg r_1(e_1)$ & $r_1 \rightarrow \neg r_2$ & She is \textbf{not} in Ranchipur. \\ \hline

\end{tabular}
}
\vspace{-3mm}
\caption{Types of counterfactuals targeted for generation.
The examples illustrate how counterfactual questions modify the semantics regarding temporal aspects ($r_1$,$r_2$) including relations and properties, for events ($e_1$,$e_2$,$e_3$).
}
\vspace{-5mm}
\label{tab:contrast_examples}
\end{table*}

